4D Generic Video Object Proposals

Many high-level video understanding methods require input in the form of object proposals. Currently, such proposals are predominantly generated with the help of networks that were trained for detecting and segmenting a set of known object classes, which limits their applicability to cases where all objects of interest are represented in the training set. This is a restriction for automotive scenarios, where unknown objects can frequently occur. We propose an approach that can reliably extract spatio-temporal object proposals for both known and unknown object categories from stereo video. Our 4D Generic Video Tubes (4D-GVT) method leverages motion cues, stereo data, and object instance segmentation to compute a compact set of video-object proposals that precisely localizes object candidates and their contours in 3D space and time. We show that given only a small amount of labeled data, our 4D-GVT proposal generator generalizes well to real-world scenarios, in which unknown categories appear. It outperforms other approaches that try to detect as many objects as possible by increasing the number of classes in the training set to several thousand.

==> KTC_stats.tex <==
\begin{center}
  \begin{table*}
  \tiny
    \begin{tabular}{l|c|r|Sc||l|c|r|Sc} %
      \textbf{Name} & \textbf{In COCO?} & \textbf{Frequency} & \textbf{Example} & \textbf{Name} & \textbf{In COCO?} & \textbf{Frequency} & \textbf{Example} \\\hline\hline%
      car & yes & \makecell{2,405\\30.04\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/car54.jpg} & building & no & \makecell{67\\0.84\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/building2340.jpg} \\\hline
      greenery & (potted plant) & \makecell{1,124\\14.04\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/greenery2791.jpg} & motorcycle & yes & \makecell{56\\0.70\%} & \cincludegraphics[height=1.0cm]{figures/class_examples/motorcycle2058.jpg} \\\hline
      window & no & \makecell{370\\4.62\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/window1089.jpg} & pole & no & \makecell{47\\0.59\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/pole23.jpg} \\\hline
      person & yes & \makecell{272\\3.40\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/person487.jpg} & trailer & no & \makecell{45\\0.56\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/trailer392.jpg} \\\hline
      road sign & (stop sign) & \makecell{192\\2.40\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/road_sign305.jpg} & wheel & no & \makecell{28\\0.35\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/wheel435.jpg} \\\hline
      fence & no & \makecell{185\\2.31\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/fence1661.jpg} & stair & no & \makecell{20\\0.25\%} & \cincludegraphics[height=0.6cm]{figures/class_examples/stair552.jpg} \\\hline
      van & no & \makecell{142\\1.77\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/van899.jpg} & license plate & no & \makecell{13\\0.16\%} & \cincludegraphics[height=0.5cm]{figures/class_examples/license_plate685.jpg} \\\hline
      bicycle & yes & \makecell{134\\1.67\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/bicycle391.jpg} & umbrella & yes & \makecell{13\\0.16\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/umbrella424.jpg} \\\hline
      wall & no & \makecell{128\\1.60\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/wall415.jpg} & bench & yes & \makecell{11\\0.14\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/bench987.jpg} \\\hline
      advertising & no & \makecell{119\\1.49\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/advertising537.jpg} & bus & yes & \makecell{10\\0.12\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/bus26.jpg} \\\hline
      rubbish bin & no & \makecell{100\\1.25\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/rubbish_bin319.jpg} & post box & no & \makecell{6\\0.08\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/post_box542.jpg} \\\hline
      gate & no & \makecell{97\\1.21\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/gate1315.jpg} & cone & no & \makecell{3\\0.04\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/cone7.jpg} \\\hline
      traffic light & yes & \makecell{87\\1.09\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/traffic_light6.jpg} & train & yes & \makecell{3\\0.04\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/train14.jpg} \\\hline
      truck & yes & \makecell{86\\1.07\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/truck962.jpg} & chair & yes & \makecell{2\\0.02\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/chair65.jpg} \\\hline
      transformer & no & \makecell{84\\1.05\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/transformer738.jpg} & animal & (dog, horse, ...) & \makecell{1\\0.01\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/animal56.jpg} \\\hline
      stone pillar & no & \makecell{76\\0.95\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/stone_pillar177.jpg} &  &  &  &  \\\hline
      cyclist & (bike, person) & \makecell{72\\0.90\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/cyclist977.jpg} & unknown & - & \makecell{1,190\\14.87\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/unknown145.jpg} \\\hline
      door & no & \makecell{72\\0.90\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/door774.jpg} & tracking error & - & \makecell{745\\9.31\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/tracking_error860.jpg}
    \end{tabular}
    \label{Tab:allClasses}
    \vspace{5pt}
    \caption{Overview of all the object classes, extracted from KITTI Raw. The frequency gives the relative amount of tracks of that class inside the dataset. License plates have been made unreadable. Note that 18 (+4 super classes) are not part of the COCO dataset.}
\end{table*}
\end{center}


==> OTC_stats.tex <==
\begin{center}
  \begin{table*}
  \tiny
    \begin{tabular}{l|c|r|Sc||l|c|r|Sc} %
      \textbf{Name} & \textbf{In COCO?} & \textbf{Frequency} & \textbf{Example} & \textbf{Name} & \textbf{In COCO?} & \textbf{Frequency} & \textbf{Example} \\\hline\hline%
      car & yes & \makecell{1894\\15.39\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/car_ox.png} & bag & no & \makecell{55\\0.45\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/bag_ox.png} \\\hline
      person & yes & \makecell{1283\\10.42\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/person_ox.png} & advertising & no & \makecell{53\\0.43\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/advertising_ox.png} \\\hline
      wheel & no & \makecell{495\\4.02\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/wheel_ox.png} & bus & yes & \makecell{39\\0.32\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/bus_ox.png} \\\hline
      bicycle & yes & \makecell{400\\3.25\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/bicycle_ox.png} & stair & no & \makecell{38\\0.31\%} & \cincludegraphics[height=0.5cm]{figures/class_examples/stair_ox.png} \\\hline
      greenery & (potted plant) & \makecell{337\\2.74\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/greenery_ox.png} & cone & no & \makecell{37\\0.30\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/cone_ox.png} \\\hline
      van & no & \makecell{293\\2.38\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/van_ox.png} & front light & no & \makecell{29\\0.24\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/front_light_ox.png} \\\hline
      back light & no & \makecell{262\\2.13\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/back_light_ox.png} & traffic light & yes & \makecell{21\\0.17\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/traffic_light_ox.png} \\\hline
      license plate & no & \makecell{248\\2.01\%} & \cincludegraphics[height=0.5cm]{figures/class_examples/license_plate_ox.png}& motorcycle & yes & \makecell{17\\0.14\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/motorcycle_ox.png} \\\hline
      road sign & (stop sign) & \makecell{220\\1.79\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/road_sign_ox.png} & transformer & no & \makecell{17\\0.14\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/transformer_ox.png} \\\hline
      wall & no & \makecell{212\\1.72\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/wall_ox.png} & side mirror & no & \makecell{15\\0.12\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/side_mirror_ox.png} \\\hline
      window & no & \makecell{211\\1.71\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/window_ox.png} & post box & no & \makecell{15\\0.12\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/post_box_ox.png} \\\hline
      fence & no & \makecell{175\\1.42\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/fence_ox.png} & building & no & \makecell{12\\0.10\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/building_ox.png}\\\hline
      cyclist & (bike, person) & \makecell{147\\1.19\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/cyclist_ox.png} & bench & yes & \makecell{11\\0.09\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/bench_ox.png} \\\hline
      stone pillar & no & \makecell{133\\1.08\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/stone_pillar_ox.png} & stroller & no & \makecell{9\\0.07\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/stroller_ox.png} \\\hline
      pole & no & \makecell{108\\0.88\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/pole_ox.png} & trailer & no & \makecell{7\\0.06\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/trailer_ox.png} \\\hline
      gate & no & \makecell{75\\0.61\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/gate_ox.png} & chair & yes & \makecell{5\\0.04\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/chair_ox.png} \\\hline
      door & no & \makecell{72\\0.58\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/door_ox.png} &  &  &  & \\\hline
      umbrella & yes & \makecell{69\\0.56\%} & \cincludegraphics[height=0.5cm]{figures/class_examples/umbrella_ox.png} & unknown & - & \makecell{4198\\34.11\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/unknown_ox.png}\\\hline
      truck & yes & \makecell{62\\0.50\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/truck_ox.png} & tracking error & - & \makecell{787\\6.39\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/tracking_error_ox.png}\\\hline
      rubbish bin & no & \makecell{62\\0.50\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/rubbishbin_ox.png} & bad lighting & - & \makecell{185\\1.50\%} & \cincludegraphics[height=0.7cm]{figures/class_examples/bad_lighting_ox2.png}
    \end{tabular}
    \label{Tab:allClassesOxford}
    \vspace{5pt}
    \caption{Overview of all the annotated track classes, extracted from Oxford. The frequency gives the relative amount of tracks of that class inside the dataset. License plates have been made unreadable. Note that 23 (+3 super classes) are not part of the COCO dataset.}
\end{table*}
\end{center}

